FAME: Feature Activation Map Explanation on Image Classification and Face Recognition

Deep Learning has revolutionized machine learning, reaching unprecedented levels of accuracy, but at the cost of reduced interpretability. Especially in image processing systems, deep networks transform local pixel information into more global concepts in a highly obscured manner. Explainable AI methods for image processing try to shed light on this issue by highlighting the regions of the image that are important for the prediction task. Among these, Class Activation Mapping (CAM) and its gradient-based variants compute attributions based on the feature map and upscale them to the image resolution, assuming that feature map locations are influenced only by underlying regions. Perturbation-based methods, such as CorrRISE, on the other hand, try to provide pixel-level attributions by perturbing the input with fixed patches and checking how the output of the network changes. In this work, we propose Feature Activation Map Explanation (FAME), which combines both worlds by using network gradients to compute changes to the input image, manipulating it in a gradient-driven way rather than using fixed patches. We apply this technique on two common tasks, image classification and face recognition, and show that CAM's above-mentioned assumption does not hold for deeper networks. We qualitatively and quantitively show that FAME produces attribution maps that are competitive state-of-the-art systems. Our code is available: {\footnotesize https://github.com/AIML-IfI/fame.}

==> figures/ARface_sim_diff_gau.tex <==
\begin{figure}[!t]
  \newcommand\img[1]{\includegraphics[width=1.3cm]{#1}}
  \centering
    \begin{tabular}{@{}c@{}c@{\,}c@{}c@{\,}c@{}c@{}}
      \img{images/ARface/gaussian/frontal_Pos_A_k5_s0.8_gal} &
      \img{images/ARface/gaussian/frontal_Pos_A_k5_s0.8_probe} &

      \img{images/ARface/gaussian/frontal_Pos_B_k11_s1.8_gal} &
      \img{images/ARface/gaussian/frontal_Pos_B_k11_s1.8_probe} &

      \img{images/ARface/gaussian/frontal_Pos_C_k15_s2.5_gal} &
      \img{images/ARface/gaussian/frontal_Pos_C_k15_s2.5_probe} \\[-.1ex]

      \img{images/ARface/gaussian/frontal_Pos_D_k25_s4.0_gal} &
      \img{images/ARface/gaussian/frontal_Pos_D_k25_s4.0_probe} &

      \img{images/ARface/gaussian/frontal_Pos_E_k49_s7.7_gal} &
      \img{images/ARface/gaussian/frontal_Pos_E_k49_s7.7_probe} &

      \img{images/ARface/gaussian/frontal_Pos_F_k81_s13_gal} &
      \img{images/ARface/gaussian/frontal_Pos_F_k81_s13_probe} \\[-.1ex]


      \img{images/ARface/gaussian/glass_Pos_A_k5_s0.8_gal} &
      \img{images/ARface/gaussian/glass_Pos_A_k5_s0.8_probe} &

      \img{images/ARface/gaussian/glass_Pos_B_k11_s1.8_gal} &
      \img{images/ARface/gaussian/glass_Pos_B_k11_s1.8_probe} &

      \img{images/ARface/gaussian/glass_Pos_C_k15_s2.5_gal} &
      \img{images/ARface/gaussian/glass_Pos_C_k15_s2.5_probe} \\[-.1ex]

      \img{images/ARface/gaussian/glass_Pos_D_k25_s4.0_gal} &
      \img{images/ARface/gaussian/glass_Pos_D_k25_s4.0_probe} &

      \img{images/ARface/gaussian/glass_Pos_E_k49_s7.7_gal} &
      \img{images/ARface/gaussian/glass_Pos_E_k49_s7.7_probe} &

      \img{images/ARface/gaussian/glass_Pos_F_k81_s13_gal} &
      \img{images/ARface/gaussian/glass_Pos_F_k81_s13_probe} \\[-.1ex]


      \img{images/ARface/gaussian/scarf_Pos_A_k5_s0.8_gal} &
      \img{images/ARface/gaussian/scarf_Pos_A_k5_s0.8_probe} &

      \img{images/ARface/gaussian/scarf_Pos_B_k11_s1.8_gal} &
      \img{images/ARface/gaussian/scarf_Pos_B_k11_s1.8_probe} &

      \img{images/ARface/gaussian/scarf_Pos_C_k15_s2.5_gal} &
      \img{images/ARface/gaussian/scarf_Pos_C_k15_s2.5_probe} \\[-.1ex]

      \img{images/ARface/gaussian/scarf_Pos_D_k25_s4.0_gal} &
      \img{images/ARface/gaussian/scarf_Pos_D_k25_s4.0_probe} &

      \img{images/ARface/gaussian/scarf_Pos_E_k49_s7.7_gal} &
      \img{images/ARface/gaussian/scarf_Pos_E_k49_s7.7_probe} &

      \img{images/ARface/gaussian/scarf_Pos_F_k81_s13_gal} &
      \img{images/ARface/gaussian/scarf_Pos_F_k81_s13_probe} \\[-.1ex]
    \end{tabular}
    % }


  \Caption[fig:lots-arface-gau]{Different Gaussian smoothing}{
    This figure shows shows the visualization results produced by the proposed FAME method under different Gaussian blur parameters, 
    where $k$ denotes the kernel size and $s$ denotes the standard deviation.
  }

\end{figure}


==> figures/ImageNET.tex <==

\begin{figure}[!t]
  \newcommand\img[1]{\includegraphics[width=0.064\textwidth]{#1}}
  \centering \tiny
    \begin{tabular}{@{\,}c@{\,}c@{\,}c@{\,}c@{\,}c@{\,}}
       & Grad-CAM & Grad-CAM-EW & HiResCAM & FAME \\[-.5ex]
      \img{images/ImageNet/single_img/ILSVRC2012_val_00002100} &
      \img{images/ImageNet/single_img/ResNet50_GradCAM_ILSVRC2012_val_00002100} &
      \img{images/ImageNet/single_img/ResNet50_GradCAMElementWise_ILSVRC2012_val_00002100} &
      \img{images/ImageNet/single_img/ResNet50_HiResCAM_ILSVRC2012_val_00002100}&
      \img{images/ImageNet/single_img/ResNet50_fame_ILSVRC2012_val_00002100}\\[-.5ex]

      \img{images/ImageNet/single_img/ILSVRC2012_val_00013733} &
      \img{images/ImageNet/single_img/ResNet50_GradCAM_ILSVRC2012_val_00013733} &
      \img{images/ImageNet/single_img/ResNet50_GradCAMElementWise_ILSVRC2012_val_00013733} &
      \img{images/ImageNet/single_img/ResNet50_HiResCAM_ILSVRC2012_val_00013733}&
      \img{images/ImageNet/single_img/ResNet50_fame_ILSVRC2012_val_00013733}\\[-.5ex]
      \end{tabular}
  \Caption[fig:activations-om-img]{ImageNet Visualization}{
    The figure shows the saliency maps generated by Grad-CAM, Grad-CAM Elementwise, HiResCAM, and the proposed FAME method using a ResNet50 model on the ImageNet classification task.

  }

\end{figure}


==> figures/fr_3.tex <==
\begin{figure*}[!t]
  \newcommand\img[1]{\includegraphics[width=0.064\textwidth]{#1}}
  \centering
  \subfloat[\label{fig:fr-arface}\textbf{ARface} -- \texttt{scarf}]{
    \begin{tabular}{@{}c@{}c@{\ }c@{}c@{\ }c@{}c@{\,}c@{}c@{\ }c@{}c@{\,}c@{}c@{\ }c@{}c@{\,}c@{}c@{}}
      \multicolumn{2}{c}{Grad-CAM} &
      \multicolumn{2}{c}{Grad-CAM-EW} &
      \multicolumn{2}{c}{CorrRISE $e_+$} &
      \multicolumn{2}{c}{CorrRISE $e_-$} &
      \multicolumn{2}{c}{FGGB $e_+$} &
      \multicolumn{2}{c}{FGGB $e_-$} &
      \multicolumn{2}{c}{FAME $e_+$} &
      \multicolumn{2}{c}{FAME $e_-$}\\
   
        \img{images/ARface/sim/Adaface_ir_18_GradCAM_frontal_Pos_0_g} &
      \img{images/ARface/sim/Adaface_ir_18_GradCAM_frontal_Pos_0_p} &
      \img{images/ARface/sim/Adaface_ir_18_GradCAMElementWise_frontal_Pos_0_g} &
      \img{images/ARface/sim/Adaface_ir_18_GradCAMElementWise_frontal_Pos_0_p}&
      \img{images/ARface/sim/Adaface_ir_18_CorrRISE_frontal_Pos_0_g_sim}&
      \img{images/ARface/sim/Adaface_ir_18_CorrRISE_frontal_Pos_0_p_sim}&
      \img{images/ARface/sim/Adaface_ir_18_CorrRISE_frontal_Pos_0_g_dissim}&
      \img{images/ARface/sim/Adaface_ir_18_CorrRISE_frontal_Pos_0_p_dissim}&
      \img{images/ARface/sim/Adaface_ir_18_fggb_frontal_Pos_0_g_sim}&
      \img{images/ARface/sim/Adaface_ir_18_fggb_frontal_Pos_0_p_sim}&
      \img{images/ARface/sim/Adaface_ir_18_fggb_frontal_Pos_0_g_dissim}&
      \img{images/ARface/sim/Adaface_ir_18_fggb_frontal_Pos_0_p_dissim}&
      \img{images/ARface/sim/Adaface_ir_18_fame_cos_frontal_Pos_0_g}&
      \img{images/ARface/sim/Adaface_ir_18_fame_cos_frontal_Pos_0_p}&
      \img{images/ARface/sim/Adaface_ir_18_fame_1-cos_frontal_Pos_0_g}&
      \img{images/ARface/sim/Adaface_ir_18_fame_1-cos_frontal_Pos_0_p}\\[-.5ex]

      \img{images/ARface/sim/Adaface_ir_50_GradCAM_frontal_Pos_0_g} &
      \img{images/ARface/sim/Adaface_ir_50_GradCAM_frontal_Pos_0_p} &
      \img{images/ARface/sim/Adaface_ir_50_GradCAMElementWise_frontal_Pos_0_g} &
      \img{images/ARface/sim/Adaface_ir_50_GradCAMElementWise_frontal_Pos_0_p}&
      \img{images/ARface/sim/Adaface_ir_50_CorrRISE_frontal_Pos_0_g_sim}&
      \img{images/ARface/sim/Adaface_ir_50_CorrRISE_frontal_Pos_0_p_sim}&
      \img{images/ARface/sim/Adaface_ir_50_CorrRISE_frontal_Pos_0_g_dissim}&
      \img{images/ARface/sim/Adaface_ir_50_CorrRISE_frontal_Pos_0_p_dissim}&
      \img{images/ARface/sim/Adaface_ir_50_fggb_frontal_Pos_0_g_sim}&
      \img{images/ARface/sim/Adaface_ir_50_fggb_frontal_Pos_0_p_sim}&
      \img{images/ARface/sim/Adaface_ir_50_fggb_frontal_Pos_0_g_dissim}&
      \img{images/ARface/sim/Adaface_ir_50_fggb_frontal_Pos_0_p_dissim}&
      \img{images/ARface/sim/Adaface_ir_50_fame_cos_frontal_Pos_0_g}&
      \img{images/ARface/sim/Adaface_ir_50_fame_cos_frontal_Pos_0_p}&
      \img{images/ARface/sim/Adaface_ir_50_fame_1-cos_frontal_Pos_0_g}&
      \img{images/ARface/sim/Adaface_ir_50_fame_1-cos_frontal_Pos_0_p}\\[-.5ex]

      \img{images/ARface/sim/Adaface_ir_101_GradCAM_frontal_Pos_0_g} &
      \img{images/ARface/sim/Adaface_ir_101_GradCAM_frontal_Pos_0_p} &
      \img{images/ARface/sim/Adaface_ir_101_GradCAMElementWise_frontal_Pos_0_g} &
      \img{images/ARface/sim/Adaface_ir_101_GradCAMElementWise_frontal_Pos_0_p}&
      \img{images/ARface/sim/Adaface_ir_101_CorrRISE_frontal_Pos_0_g_sim}&
      \img{images/ARface/sim/Adaface_ir_101_CorrRISE_frontal_Pos_0_p_sim}&
      \img{images/ARface/sim/Adaface_ir_101_CorrRISE_frontal_Pos_0_g_dissim}&
      \img{images/ARface/sim/Adaface_ir_101_CorrRISE_frontal_Pos_0_p_dissim}&
      \img{images/ARface/sim/Adaface_ir_101_fggb_frontal_Pos_0_g_sim}&
      \img{images/ARface/sim/Adaface_ir_101_fggb_frontal_Pos_0_p_sim}&
      \img{images/ARface/sim/Adaface_ir_101_fggb_frontal_Pos_0_g_dissim}&
      \img{images/ARface/sim/Adaface_ir_101_fggb_frontal_Pos_0_p_dissim}&
      \img{images/ARface/sim/Adaface_ir_101_fame_cos_frontal_Pos_0_g}&
      \img{images/ARface/sim/Adaface_ir_101_fame_cos_frontal_Pos_0_p}&
      \img{images/ARface/sim/Adaface_ir_101_fame_1-cos_frontal_Pos_0_g}&
      \img{images/ARface/sim/Adaface_ir_101_fame_1-cos_frontal_Pos_0_p}\\


      \img{images/ARface/sim/Adaface_ir_18_GradCAM_glass_Pos_5_g} &
      \img{images/ARface/sim/Adaface_ir_18_GradCAM_glass_Pos_5_p} &
      \img{images/ARface/sim/Adaface_ir_18_GradCAMElementWise_glass_Pos_5_g} &
      \img{images/ARface/sim/Adaface_ir_18_GradCAMElementWise_glass_Pos_5_p}&
      \img{images/ARface/sim/Adaface_ir_18_CorrRISE_glass_Pos_5_g_sim}&
      \img{images/ARface/sim/Adaface_ir_18_CorrRISE_glass_Pos_5_p_sim}&
      \img{images/ARface/sim/Adaface_ir_18_CorrRISE_glass_Pos_5_g_dissim}&
      \img{images/ARface/sim/Adaface_ir_18_CorrRISE_glass_Pos_5_p_dissim}&
      \img{images/ARface/sim/Adaface_ir_18_fggb_glass_Pos_5_g_sim}&
      \img{images/ARface/sim/Adaface_ir_18_fggb_glass_Pos_5_p_sim}&
      \img{images/ARface/sim/Adaface_ir_18_fggb_glass_Pos_5_g_dissim}&
      \img{images/ARface/sim/Adaface_ir_18_fggb_glass_Pos_5_p_dissim}&
      \img{images/ARface/sim/Adaface_ir_18_fame_cos_glass_Pos_5_g}&
      \img{images/ARface/sim/Adaface_ir_18_fame_cos_glass_Pos_5_p}&
      \img{images/ARface/sim/Adaface_ir_18_fame_1-cos_glass_Pos_5_g}&
      \img{images/ARface/sim/Adaface_ir_18_fame_1-cos_glass_Pos_5_p}\\[-.5ex]

      \img{images/ARface/sim/Adaface_ir_50_GradCAM_glass_Pos_5_g} &
      \img{images/ARface/sim/Adaface_ir_50_GradCAM_glass_Pos_5_p} &
      \img{images/ARface/sim/Adaface_ir_50_GradCAMElementWise_glass_Pos_5_g} &
      \img{images/ARface/sim/Adaface_ir_50_GradCAMElementWise_glass_Pos_5_p}&
      \img{images/ARface/sim/Adaface_ir_50_CorrRISE_glass_Pos_5_g_sim}&
      \img{images/ARface/sim/Adaface_ir_50_CorrRISE_glass_Pos_5_p_sim}&
      \img{images/ARface/sim/Adaface_ir_50_CorrRISE_glass_Pos_5_g_dissim}&
      \img{images/ARface/sim/Adaface_ir_50_CorrRISE_glass_Pos_5_p_dissim}&
      \img{images/ARface/sim/Adaface_ir_50_fggb_glass_Pos_5_g_sim}&
      \img{images/ARface/sim/Adaface_ir_50_fggb_glass_Pos_5_p_sim}&
      \img{images/ARface/sim/Adaface_ir_50_fggb_glass_Pos_5_g_dissim}&
      \img{images/ARface/sim/Adaface_ir_50_fggb_glass_Pos_5_p_dissim}&
      \img{images/ARface/sim/Adaface_ir_50_fame_cos_glass_Pos_5_g}&
      \img{images/ARface/sim/Adaface_ir_50_fame_cos_glass_Pos_5_p}&
      \img{images/ARface/sim/Adaface_ir_50_fame_1-cos_glass_Pos_5_g}&
      \img{images/ARface/sim/Adaface_ir_50_fame_1-cos_glass_Pos_5_p}\\[-.5ex]

      \img{images/ARface/sim/Adaface_ir_101_GradCAM_glass_Pos_5_g} &
      \img{images/ARface/sim/Adaface_ir_101_GradCAM_glass_Pos_5_p} &
      \img{images/ARface/sim/Adaface_ir_101_GradCAMElementWise_glass_Pos_5_g} &
      \img{images/ARface/sim/Adaface_ir_101_GradCAMElementWise_glass_Pos_5_p}&
      \img{images/ARface/sim/Adaface_ir_101_CorrRISE_glass_Pos_5_g_sim}&
      \img{images/ARface/sim/Adaface_ir_101_CorrRISE_glass_Pos_5_p_sim}&
      \img{images/ARface/sim/Adaface_ir_101_CorrRISE_glass_Pos_5_g_dissim}&
      \img{images/ARface/sim/Adaface_ir_101_CorrRISE_glass_Pos_5_p_dissim}&
      \img{images/ARface/sim/Adaface_ir_101_fggb_glass_Pos_5_g_sim}&
      \img{images/ARface/sim/Adaface_ir_101_fggb_glass_Pos_5_p_sim}&
      \img{images/ARface/sim/Adaface_ir_101_fggb_glass_Pos_5_g_dissim}&
      \img{images/ARface/sim/Adaface_ir_101_fggb_glass_Pos_5_p_dissim}&
      \img{images/ARface/sim/Adaface_ir_101_fame_cos_glass_Pos_5_g}&
      \img{images/ARface/sim/Adaface_ir_101_fame_cos_glass_Pos_5_p}&
      \img{images/ARface/sim/Adaface_ir_101_fame_1-cos_glass_Pos_5_g}&
      \img{images/ARface/sim/Adaface_ir_101_fame_1-cos_glass_Pos_5_p}\\
      
      
      \img{images/ARface/sim/Adaface_ir_18_GradCAM_scarf_Pos_6_g} &
      \img{images/ARface/sim/Adaface_ir_18_GradCAM_scarf_Pos_6_p} &
      \img{images/ARface/sim/Adaface_ir_18_GradCAMElementWise_scarf_Pos_6_g} &
      \img{images/ARface/sim/Adaface_ir_18_GradCAMElementWise_scarf_Pos_6_p}&
      \img{images/ARface/sim/Adaface_ir_18_CorrRISE_scarf_Pos_6_g_sim}&
      \img{images/ARface/sim/Adaface_ir_18_CorrRISE_scarf_Pos_6_p_sim}&
      \img{images/ARface/sim/Adaface_ir_18_CorrRISE_scarf_Pos_6_g_dissim}&
      \img{images/ARface/sim/Adaface_ir_18_CorrRISE_scarf_Pos_6_p_dissim}&
      \img{images/ARface/sim/Adaface_ir_18_fggb_scarf_Pos_6_g_sim}&
      \img{images/ARface/sim/Adaface_ir_18_fggb_scarf_Pos_6_p_sim}&
      \img{images/ARface/sim/Adaface_ir_18_fggb_scarf_Pos_6_g_dissim}&
      \img{images/ARface/sim/Adaface_ir_18_fggb_scarf_Pos_6_p_dissim}&
      \img{images/ARface/sim/Adaface_ir_18_fame_cos_scarf_Pos_6_g}&
      \img{images/ARface/sim/Adaface_ir_18_fame_cos_scarf_Pos_6_p}&
      \img{images/ARface/sim/Adaface_ir_18_fame_1-cos_scarf_Pos_6_g}&
      \img{images/ARface/sim/Adaface_ir_18_fame_1-cos_scarf_Pos_6_p}\\[-.5ex]

      \img{images/ARface/sim/Adaface_ir_50_GradCAM_scarf_Pos_6_g} &
      \img{images/ARface/sim/Adaface_ir_50_GradCAM_scarf_Pos_6_p} &
      \img{images/ARface/sim/Adaface_ir_50_GradCAMElementWise_scarf_Pos_6_g} &
      \img{images/ARface/sim/Adaface_ir_50_GradCAMElementWise_scarf_Pos_6_p}&
      \img{images/ARface/sim/Adaface_ir_50_CorrRISE_scarf_Pos_6_g_sim}&
      \img{images/ARface/sim/Adaface_ir_50_CorrRISE_scarf_Pos_6_p_sim}&
      \img{images/ARface/sim/Adaface_ir_50_CorrRISE_scarf_Pos_6_g_dissim}&
      \img{images/ARface/sim/Adaface_ir_50_CorrRISE_scarf_Pos_6_p_dissim}&
      \img{images/ARface/sim/Adaface_ir_50_fggb_scarf_Pos_6_g_sim}&
      \img{images/ARface/sim/Adaface_ir_50_fggb_scarf_Pos_6_p_sim}&
      \img{images/ARface/sim/Adaface_ir_50_fggb_scarf_Pos_6_g_dissim}&
      \img{images/ARface/sim/Adaface_ir_50_fggb_scarf_Pos_6_p_dissim}&
      \img{images/ARface/sim/Adaface_ir_50_fame_cos_scarf_Pos_6_g}&
      \img{images/ARface/sim/Adaface_ir_50_fame_cos_scarf_Pos_6_p}&
      \img{images/ARface/sim/Adaface_ir_50_fame_1-cos_scarf_Pos_6_g}&
      \img{images/ARface/sim/Adaface_ir_50_fame_1-cos_scarf_Pos_6_p}\\[-.5ex]


      \img{images/ARface/sim/Adaface_ir_101_GradCAM_scarf_Pos_6_g} &
      \img{images/ARface/sim/Adaface_ir_101_GradCAM_scarf_Pos_6_p} &
      \img{images/ARface/sim/Adaface_ir_101_GradCAMElementWise_scarf_Pos_6_g} &
      \img{images/ARface/sim/Adaface_ir_101_GradCAMElementWise_scarf_Pos_6_p}&
      \img{images/ARface/sim/Adaface_ir_101_CorrRISE_scarf_Pos_6_g_sim}&
      \img{images/ARface/sim/Adaface_ir_101_CorrRISE_scarf_Pos_6_p_sim}&
      \img{images/ARface/sim/Adaface_ir_101_CorrRISE_scarf_Pos_6_g_dissim}&
      \img{images/ARface/sim/Adaface_ir_101_CorrRISE_scarf_Pos_6_p_dissim}&
      \img{images/ARface/sim/Adaface_ir_101_fggb_scarf_Pos_6_g_sim}&
      \img{images/ARface/sim/Adaface_ir_101_fggb_scarf_Pos_6_p_sim}&
      \img{images/ARface/sim/Adaface_ir_101_fggb_scarf_Pos_6_g_dissim}&
      \img{images/ARface/sim/Adaface_ir_101_fggb_scarf_Pos_6_p_dissim}&
      \img{images/ARface/sim/Adaface_ir_101_fame_cos_scarf_Pos_6_g}&
      \img{images/ARface/sim/Adaface_ir_101_fame_cos_scarf_Pos_6_p}&
      \img{images/ARface/sim/Adaface_ir_101_fame_1-cos_scarf_Pos_6_g}&
      \img{images/ARface/sim/Adaface_ir_101_fame_1-cos_scarf_Pos_6_p}\\[-.5ex]
      \end{tabular}
      }

  \subfloat[\label{fig:fr-scface}\textbf{SCface} -- \texttt{medium}]{
    \begin{tabular}{@{}c@{}c@{\ }c@{}c@{\ }c@{}c@{\,}c@{}c@{\ }c@{}c@{\,}c@{}c@{\ }c@{}c@{\,}c@{}c@{}}
      
      \img{images/SCface/sim/Adaface_ir_18_GradCAM_close_Pos_23_g} &
      \img{images/SCface/sim/Adaface_ir_18_GradCAM_close_Pos_23_p} &
      \img{images/SCface/sim/Adaface_ir_18_GradCAMElementWise_close_Pos_23_g} &
      \img{images/SCface/sim/Adaface_ir_18_GradCAMElementWise_close_Pos_23_p}&
      \img{images/SCface/sim/Adaface_ir_18_CorrRISE_close_Pos_23_g_sim}&
      \img{images/SCface/sim/Adaface_ir_18_CorrRISE_close_Pos_23_p_sim}&
      \img{images/SCface/sim/Adaface_ir_18_CorrRISE_close_Pos_23_g_dissim}&
      \img{images/SCface/sim/Adaface_ir_18_CorrRISE_close_Pos_23_p_dissim}&
      \img{images/SCface/sim/Adaface_ir_18_fggb_close_Pos_23_g_sim}&
      \img{images/SCface/sim/Adaface_ir_18_fggb_close_Pos_23_p_sim}&
      \img{images/SCface/sim/Adaface_ir_18_fggb_close_Pos_23_g_dissim}&
      \img{images/SCface/sim/Adaface_ir_18_fggb_close_Pos_23_p_dissim}&
      \img{images/SCface/sim/Adaface_ir_18_fame_cos_close_Pos_23_g}&
      \img{images/SCface/sim/Adaface_ir_18_fame_cos_close_Pos_23_p}&
      \img{images/SCface/sim/Adaface_ir_18_fame_1-cos_close_Pos_23_g}&
      \img{images/SCface/sim/Adaface_ir_18_fame_1-cos_close_Pos_23_p}\\[-.5ex]

      \img{images/SCface/sim/Adaface_ir_50_GradCAM_close_Pos_23_g} &
      \img{images/SCface/sim/Adaface_ir_50_GradCAM_close_Pos_23_p} &
      \img{images/SCface/sim/Adaface_ir_50_GradCAMElementWise_close_Pos_23_g} &
      \img{images/SCface/sim/Adaface_ir_50_GradCAMElementWise_close_Pos_23_p}&
      \img{images/SCface/sim/Adaface_ir_50_CorrRISE_close_Pos_23_g_sim}&
      \img{images/SCface/sim/Adaface_ir_50_CorrRISE_close_Pos_23_p_sim}&
      \img{images/SCface/sim/Adaface_ir_50_CorrRISE_close_Pos_23_g_dissim}&
      \img{images/SCface/sim/Adaface_ir_50_CorrRISE_close_Pos_23_p_dissim}&
      \img{images/SCface/sim/Adaface_ir_50_fggb_close_Pos_23_g_sim}&
      \img{images/SCface/sim/Adaface_ir_50_fggb_close_Pos_23_p_sim}&
      \img{images/SCface/sim/Adaface_ir_50_fggb_close_Pos_23_g_dissim}&
      \img{images/SCface/sim/Adaface_ir_50_fggb_close_Pos_23_p_dissim}&
      \img{images/SCface/sim/Adaface_ir_50_fame_cos_close_Pos_23_g}&
      \img{images/SCface/sim/Adaface_ir_50_fame_cos_close_Pos_23_p}&
      \img{images/SCface/sim/Adaface_ir_50_fame_1-cos_close_Pos_23_g}&
      \img{images/SCface/sim/Adaface_ir_50_fame_1-cos_close_Pos_23_p}\\[-.5ex]

      \img{images/SCface/sim/Adaface_ir_101_GradCAM_close_Pos_23_g} &
      \img{images/SCface/sim/Adaface_ir_101_GradCAM_close_Pos_23_p} &
      \img{images/SCface/sim/Adaface_ir_101_GradCAMElementWise_close_Pos_23_g} &
      \img{images/SCface/sim/Adaface_ir_101_GradCAMElementWise_close_Pos_23_p}&
      \img{images/SCface/sim/Adaface_ir_101_CorrRISE_close_Pos_23_g_sim}&
      \img{images/SCface/sim/Adaface_ir_101_CorrRISE_close_Pos_23_p_sim}&
      \img{images/SCface/sim/Adaface_ir_101_CorrRISE_close_Pos_23_g_dissim}&
      \img{images/SCface/sim/Adaface_ir_101_CorrRISE_close_Pos_23_p_dissim}&
      \img{images/SCface/sim/Adaface_ir_101_fggb_close_Pos_23_g_sim}&
      \img{images/SCface/sim/Adaface_ir_101_fggb_close_Pos_23_p_sim}&
      \img{images/SCface/sim/Adaface_ir_101_fggb_close_Pos_23_g_dissim}&
      \img{images/SCface/sim/Adaface_ir_101_fggb_close_Pos_23_p_dissim}&
      \img{images/SCface/sim/Adaface_ir_101_fame_cos_close_Pos_23_g}&
      \img{images/SCface/sim/Adaface_ir_101_fame_cos_close_Pos_23_p}&
      \img{images/SCface/sim/Adaface_ir_101_fame_1-cos_close_Pos_23_g}&
      \img{images/SCface/sim/Adaface_ir_101_fame_1-cos_close_Pos_23_p}\\


      \img{images/SCface/sim/Adaface_ir_18_GradCAM_medium_Pos_17_g} &
      \img{images/SCface/sim/Adaface_ir_18_GradCAM_medium_Pos_17_p} &
      \img{images/SCface/sim/Adaface_ir_18_GradCAMElementWise_medium_Pos_17_g} &
      \img{images/SCface/sim/Adaface_ir_18_GradCAMElementWise_medium_Pos_17_p}&
      \img{images/SCface/sim/Adaface_ir_18_CorrRISE_medium_Pos_17_g_sim}&
      \img{images/SCface/sim/Adaface_ir_18_CorrRISE_medium_Pos_17_p_sim}&
      \img{images/SCface/sim/Adaface_ir_18_CorrRISE_medium_Pos_17_g_dissim}&
      \img{images/SCface/sim/Adaface_ir_18_CorrRISE_medium_Pos_17_p_dissim}&
      \img{images/SCface/sim/Adaface_ir_18_fggb_medium_Pos_17_g_sim}&
      \img{images/SCface/sim/Adaface_ir_18_fggb_medium_Pos_17_p_sim}&
      \img{images/SCface/sim/Adaface_ir_18_fggb_medium_Pos_17_g_dissim}&
      \img{images/SCface/sim/Adaface_ir_18_fggb_medium_Pos_17_p_dissim}&
      \img{images/SCface/sim/Adaface_ir_18_fame_cos_medium_Pos_17_g}&
      \img{images/SCface/sim/Adaface_ir_18_fame_cos_medium_Pos_17_p}&
      \img{images/SCface/sim/Adaface_ir_18_fame_1-cos_medium_Pos_17_g}&
      \img{images/SCface/sim/Adaface_ir_18_fame_1-cos_medium_Pos_17_p}\\[-.5ex]

      \img{images/SCface/sim/Adaface_ir_50_GradCAM_medium_Pos_17_g} &
      \img{images/SCface/sim/Adaface_ir_50_GradCAM_medium_Pos_17_p} &
      \img{images/SCface/sim/Adaface_ir_50_GradCAMElementWise_medium_Pos_17_g} &
      \img{images/SCface/sim/Adaface_ir_50_GradCAMElementWise_medium_Pos_17_p}&
      \img{images/SCface/sim/Adaface_ir_50_CorrRISE_medium_Pos_17_g_sim}&
      \img{images/SCface/sim/Adaface_ir_50_CorrRISE_medium_Pos_17_p_sim}&
      \img{images/SCface/sim/Adaface_ir_50_CorrRISE_medium_Pos_17_g_dissim}&
      \img{images/SCface/sim/Adaface_ir_50_CorrRISE_medium_Pos_17_p_dissim}&
      \img{images/SCface/sim/Adaface_ir_50_fggb_medium_Pos_17_g_sim}&
      \img{images/SCface/sim/Adaface_ir_50_fggb_medium_Pos_17_p_sim}&
      \img{images/SCface/sim/Adaface_ir_50_fggb_medium_Pos_17_g_dissim}&
      \img{images/SCface/sim/Adaface_ir_50_fggb_medium_Pos_17_p_dissim}&
      \img{images/SCface/sim/Adaface_ir_50_fame_cos_medium_Pos_17_g}&
      \img{images/SCface/sim/Adaface_ir_50_fame_cos_medium_Pos_17_p}&
      \img{images/SCface/sim/Adaface_ir_50_fame_1-cos_medium_Pos_17_g}&
      \img{images/SCface/sim/Adaface_ir_50_fame_1-cos_medium_Pos_17_p}\\[-.5ex]

      \img{images/SCface/sim/Adaface_ir_101_GradCAM_medium_Pos_17_g} &
      \img{images/SCface/sim/Adaface_ir_101_GradCAM_medium_Pos_17_p} &
      \img{images/SCface/sim/Adaface_ir_101_GradCAMElementWise_medium_Pos_17_g} &
      \img{images/SCface/sim/Adaface_ir_101_GradCAMElementWise_medium_Pos_17_p}&
      \img{images/SCface/sim/Adaface_ir_101_CorrRISE_medium_Pos_17_g_sim}&
      \img{images/SCface/sim/Adaface_ir_101_CorrRISE_medium_Pos_17_p_sim}&
      \img{images/SCface/sim/Adaface_ir_101_CorrRISE_medium_Pos_17_g_dissim}&
      \img{images/SCface/sim/Adaface_ir_101_CorrRISE_medium_Pos_17_p_dissim}&
      \img{images/SCface/sim/Adaface_ir_101_fggb_medium_Pos_17_g_sim}&
      \img{images/SCface/sim/Adaface_ir_101_fggb_medium_Pos_17_p_sim}&
      \img{images/SCface/sim/Adaface_ir_101_fggb_medium_Pos_17_g_dissim}&
      \img{images/SCface/sim/Adaface_ir_101_fggb_medium_Pos_17_p_dissim}&
      \img{images/SCface/sim/Adaface_ir_101_fame_cos_medium_Pos_17_g}&
      \img{images/SCface/sim/Adaface_ir_101_fame_cos_medium_Pos_17_p}&
      \img{images/SCface/sim/Adaface_ir_101_fame_1-cos_medium_Pos_17_g}&
      \img{images/SCface/sim/Adaface_ir_101_fame_1-cos_medium_Pos_17_p}\\
      
      
      \img{images/SCface/sim/Adaface_ir_18_GradCAM_far_Pos_44_g} &
      \img{images/SCface/sim/Adaface_ir_18_GradCAM_far_Pos_44_p} &
      \img{images/SCface/sim/Adaface_ir_18_GradCAMElementWise_far_Pos_44_g} &
      \img{images/SCface/sim/Adaface_ir_18_GradCAMElementWise_far_Pos_44_p}&
      \img{images/SCface/sim/Adaface_ir_18_CorrRISE_far_Pos_44_g_sim}&
      \img{images/SCface/sim/Adaface_ir_18_CorrRISE_far_Pos_44_p_sim}&
      \img{images/SCface/sim/Adaface_ir_18_CorrRISE_far_Pos_44_g_dissim}&
      \img{images/SCface/sim/Adaface_ir_18_CorrRISE_far_Pos_44_p_dissim}&
      \img{images/SCface/sim/Adaface_ir_18_fggb_far_Pos_44_g_sim}&
      \img{images/SCface/sim/Adaface_ir_18_fggb_far_Pos_44_p_sim}&
      \img{images/SCface/sim/Adaface_ir_18_fggb_far_Pos_44_g_dissim}&
      \img{images/SCface/sim/Adaface_ir_18_fggb_far_Pos_44_p_dissim}&
      \img{images/SCface/sim/Adaface_ir_18_fame_cos_far_Pos_44_g}&
      \img{images/SCface/sim/Adaface_ir_18_fame_cos_far_Pos_44_p}&
      \img{images/SCface/sim/Adaface_ir_18_fame_1-cos_far_Pos_44_g}&
      \img{images/SCface/sim/Adaface_ir_18_fame_1-cos_far_Pos_44_p}\\[-.5ex]

      \img{images/SCface/sim/Adaface_ir_50_GradCAM_far_Pos_44_g} &
      \img{images/SCface/sim/Adaface_ir_50_GradCAM_far_Pos_44_p} &
      \img{images/SCface/sim/Adaface_ir_50_GradCAMElementWise_far_Pos_44_g} &
      \img{images/SCface/sim/Adaface_ir_50_GradCAMElementWise_far_Pos_44_p}&
      \img{images/SCface/sim/Adaface_ir_50_CorrRISE_far_Pos_44_g_sim}&
      \img{images/SCface/sim/Adaface_ir_50_CorrRISE_far_Pos_44_p_sim}&
      \img{images/SCface/sim/Adaface_ir_50_CorrRISE_far_Pos_44_g_dissim}&
      \img{images/SCface/sim/Adaface_ir_50_CorrRISE_far_Pos_44_p_dissim}&
      \img{images/SCface/sim/Adaface_ir_50_fggb_far_Pos_44_g_sim}&
      \img{images/SCface/sim/Adaface_ir_50_fggb_far_Pos_44_p_sim}&
      \img{images/SCface/sim/Adaface_ir_50_fggb_far_Pos_44_g_dissim}&
      \img{images/SCface/sim/Adaface_ir_50_fggb_far_Pos_44_p_dissim}&
      \img{images/SCface/sim/Adaface_ir_50_fame_cos_far_Pos_44_g}&
      \img{images/SCface/sim/Adaface_ir_50_fame_cos_far_Pos_44_p}&
      \img{images/SCface/sim/Adaface_ir_50_fame_1-cos_far_Pos_44_g}&
      \img{images/SCface/sim/Adaface_ir_50_fame_1-cos_far_Pos_44_p}\\[-.5ex]


      \img{images/SCface/sim/Adaface_ir_101_GradCAM_far_Pos_44_g} &
      \img{images/SCface/sim/Adaface_ir_101_GradCAM_far_Pos_44_p} &
      \img{images/SCface/sim/Adaface_ir_101_GradCAMElementWise_far_Pos_44_g} &
      \img{images/SCface/sim/Adaface_ir_101_GradCAMElementWise_far_Pos_44_p}&
      \img{images/SCface/sim/Adaface_ir_101_CorrRISE_far_Pos_44_g_sim}&
      \img{images/SCface/sim/Adaface_ir_101_CorrRISE_far_Pos_44_p_sim}&
      \img{images/SCface/sim/Adaface_ir_101_CorrRISE_far_Pos_44_g_dissim}&
      \img{images/SCface/sim/Adaface_ir_101_CorrRISE_far_Pos_44_p_dissim}&
      \img{images/SCface/sim/Adaface_ir_101_fggb_far_Pos_44_g_sim}&
      \img{images/SCface/sim/Adaface_ir_101_fggb_far_Pos_44_p_sim}&
      \img{images/SCface/sim/Adaface_ir_101_fggb_far_Pos_44_g_dissim}&
      \img{images/SCface/sim/Adaface_ir_101_fggb_far_Pos_44_p_dissim}&
      \img{images/SCface/sim/Adaface_ir_101_fame_cos_far_Pos_44_g}&
      \img{images/SCface/sim/Adaface_ir_101_fame_cos_far_Pos_44_p}&
      \img{images/SCface/sim/Adaface_ir_101_fame_1-cos_far_Pos_44_g}&
      \img{images/SCface/sim/Adaface_ir_101_fame_1-cos_far_Pos_44_p}\\[-.5ex]
      \end{tabular}
      }


    \subfloat[\label{fig:fr-cfp}\textbf{CFP} -- \texttt{FP}]{
    \begin{tabular}{@{}c@{}c@{\ }c@{}c@{\ }c@{}c@{\,}c@{}c@{\ }c@{}c@{\,}c@{}c@{\ }c@{}c@{\,}c@{}c@{}}
      
      \img{images/CFP/sim/Adaface_ir_18_GradCAM_01FF_Pos_4_g} &
      \img{images/CFP/sim/Adaface_ir_18_GradCAM_01FF_Pos_4_p} &
      \img{images/CFP/sim/Adaface_ir_18_GradCAMElementWise_01FF_Pos_4_g} &
      \img{images/CFP/sim/Adaface_ir_18_GradCAMElementWise_01FF_Pos_4_p}&
      \img{images/CFP/sim/Adaface_ir_18_CorrRISE_01FF_Pos_4_g_sim}&
      \img{images/CFP/sim/Adaface_ir_18_CorrRISE_01FF_Pos_4_p_sim}&
      \img{images/CFP/sim/Adaface_ir_18_CorrRISE_01FF_Pos_4_g_dissim}&
      \img{images/CFP/sim/Adaface_ir_18_CorrRISE_01FF_Pos_4_p_dissim}&
      \img{images/CFP/sim/Adaface_ir_18_fggb_01FF_Pos_4_g_sim}&
      \img{images/CFP/sim/Adaface_ir_18_fggb_01FF_Pos_4_p_sim}&
      \img{images/CFP/sim/Adaface_ir_18_fggb_01FF_Pos_4_g_dissim}&
      \img{images/CFP/sim/Adaface_ir_18_fggb_01FF_Pos_4_p_dissim}&
      \img{images/CFP/sim/Adaface_ir_18_fame_cos_01FF_Pos_4_g}&
      \img{images/CFP/sim/Adaface_ir_18_fame_cos_01FF_Pos_4_p}&
      \img{images/CFP/sim/Adaface_ir_18_fame_1-cos_01FF_Pos_4_g}&
      \img{images/CFP/sim/Adaface_ir_18_fame_1-cos_01FF_Pos_4_p}\\[-.5ex]

      \img{images/CFP/sim/Adaface_ir_50_GradCAM_01FF_Pos_4_g} &
      \img{images/CFP/sim/Adaface_ir_50_GradCAM_01FF_Pos_4_p} &
      \img{images/CFP/sim/Adaface_ir_50_GradCAMElementWise_01FF_Pos_4_g} &
      \img{images/CFP/sim/Adaface_ir_50_GradCAMElementWise_01FF_Pos_4_p}&
      \img{images/CFP/sim/Adaface_ir_50_CorrRISE_01FF_Pos_4_g_sim}&
      \img{images/CFP/sim/Adaface_ir_50_CorrRISE_01FF_Pos_4_p_sim}&
      \img{images/CFP/sim/Adaface_ir_50_CorrRISE_01FF_Pos_4_g_dissim}&
      \img{images/CFP/sim/Adaface_ir_50_CorrRISE_01FF_Pos_4_p_dissim}&
      \img{images/CFP/sim/Adaface_ir_50_fggb_01FF_Pos_4_g_sim}&
      \img{images/CFP/sim/Adaface_ir_50_fggb_01FF_Pos_4_p_sim}&
      \img{images/CFP/sim/Adaface_ir_50_fggb_01FF_Pos_4_g_dissim}&
      \img{images/CFP/sim/Adaface_ir_50_fggb_01FF_Pos_4_p_dissim}&
      \img{images/CFP/sim/Adaface_ir_50_fame_cos_01FF_Pos_4_g}&
      \img{images/CFP/sim/Adaface_ir_50_fame_cos_01FF_Pos_4_p}&
      \img{images/CFP/sim/Adaface_ir_50_fame_1-cos_01FF_Pos_4_g}&
      \img{images/CFP/sim/Adaface_ir_50_fame_1-cos_01FF_Pos_4_p}\\[-.5ex]

      \img{images/CFP/sim/Adaface_ir_101_GradCAM_01FF_Pos_4_g} &
      \img{images/CFP/sim/Adaface_ir_101_GradCAM_01FF_Pos_4_p} &
      \img{images/CFP/sim/Adaface_ir_101_GradCAMElementWise_01FF_Pos_4_g} &
      \img{images/CFP/sim/Adaface_ir_101_GradCAMElementWise_01FF_Pos_4_p}&
      \img{images/CFP/sim/Adaface_ir_101_CorrRISE_01FF_Pos_4_g_sim}&
      \img{images/CFP/sim/Adaface_ir_101_CorrRISE_01FF_Pos_4_p_sim}&
      \img{images/CFP/sim/Adaface_ir_101_CorrRISE_01FF_Pos_4_g_dissim}&
      \img{images/CFP/sim/Adaface_ir_101_CorrRISE_01FF_Pos_4_p_dissim}&
      \img{images/CFP/sim/Adaface_ir_101_fggb_01FF_Pos_4_g_sim}&
      \img{images/CFP/sim/Adaface_ir_101_fggb_01FF_Pos_4_p_sim}&
      \img{images/CFP/sim/Adaface_ir_101_fggb_01FF_Pos_4_g_dissim}&
      \img{images/CFP/sim/Adaface_ir_101_fggb_01FF_Pos_4_p_dissim}&
      \img{images/CFP/sim/Adaface_ir_101_fame_cos_01FF_Pos_4_g}&
      \img{images/CFP/sim/Adaface_ir_101_fame_cos_01FF_Pos_4_p}&
      \img{images/CFP/sim/Adaface_ir_101_fame_1-cos_01FF_Pos_4_g}&
      \img{images/CFP/sim/Adaface_ir_101_fame_1-cos_01FF_Pos_4_p}\\


      \img{images/CFP/sim/Adaface_ir_18_GradCAM_01FP_Pos_505_g} &
      \img{images/CFP/sim/Adaface_ir_18_GradCAM_01FP_Pos_505_p} &
      \img{images/CFP/sim/Adaface_ir_18_GradCAMElementWise_01FP_Pos_505_g} &
      \img{images/CFP/sim/Adaface_ir_18_GradCAMElementWise_01FP_Pos_505_p}&
      \img{images/CFP/sim/Adaface_ir_18_CorrRISE_01FP_Pos_505_g_sim}&
      \img{images/CFP/sim/Adaface_ir_18_CorrRISE_01FP_Pos_505_p_sim}&
      \img{images/CFP/sim/Adaface_ir_18_CorrRISE_01FP_Pos_505_g_dissim}&
      \img{images/CFP/sim/Adaface_ir_18_CorrRISE_01FP_Pos_505_p_dissim}&
      \img{images/CFP/sim/Adaface_ir_18_fggb_01FP_Pos_505_g_sim}&
      \img{images/CFP/sim/Adaface_ir_18_fggb_01FP_Pos_505_p_sim}&
      \img{images/CFP/sim/Adaface_ir_18_fggb_01FP_Pos_505_g_dissim}&
      \img{images/CFP/sim/Adaface_ir_18_fggb_01FP_Pos_505_p_dissim}&      
      \img{images/CFP/sim/Adaface_ir_18_fame_cos_01FP_Pos_505_g}&
      \img{images/CFP/sim/Adaface_ir_18_fame_cos_01FP_Pos_505_p}&
      \img{images/CFP/sim/Adaface_ir_18_fame_1-cos_01FP_Pos_505_g}&
      \img{images/CFP/sim/Adaface_ir_18_fame_1-cos_01FP_Pos_505_p}\\[-.5ex]

      \img{images/CFP/sim/Adaface_ir_50_GradCAM_01FP_Pos_505_g} &
      \img{images/CFP/sim/Adaface_ir_50_GradCAM_01FP_Pos_505_p} &
      \img{images/CFP/sim/Adaface_ir_50_GradCAMElementWise_01FP_Pos_505_g} &
      \img{images/CFP/sim/Adaface_ir_50_GradCAMElementWise_01FP_Pos_505_p}&
      \img{images/CFP/sim/Adaface_ir_50_CorrRISE_01FP_Pos_505_g_sim}&
      \img{images/CFP/sim/Adaface_ir_50_CorrRISE_01FP_Pos_505_p_sim}&
      \img{images/CFP/sim/Adaface_ir_50_CorrRISE_01FP_Pos_505_g_dissim}&
      \img{images/CFP/sim/Adaface_ir_50_CorrRISE_01FP_Pos_505_p_dissim}&
      \img{images/CFP/sim/Adaface_ir_50_fggb_01FP_Pos_505_g_sim}&
      \img{images/CFP/sim/Adaface_ir_50_fggb_01FP_Pos_505_p_sim}&
      \img{images/CFP/sim/Adaface_ir_50_fggb_01FP_Pos_505_g_dissim}&
      \img{images/CFP/sim/Adaface_ir_50_fggb_01FP_Pos_505_p_dissim}&      
      \img{images/CFP/sim/Adaface_ir_50_fame_cos_01FP_Pos_505_g}&
      \img{images/CFP/sim/Adaface_ir_50_fame_cos_01FP_Pos_505_p}&
      \img{images/CFP/sim/Adaface_ir_50_fame_1-cos_01FP_Pos_505_g}&
      \img{images/CFP/sim/Adaface_ir_50_fame_1-cos_01FP_Pos_505_p}\\[-.5ex]

      \img{images/CFP/sim/Adaface_ir_101_GradCAM_01FP_Pos_505_g} &
      \img{images/CFP/sim/Adaface_ir_101_GradCAM_01FP_Pos_505_p} &
      \img{images/CFP/sim/Adaface_ir_101_GradCAMElementWise_01FP_Pos_505_g} &
      \img{images/CFP/sim/Adaface_ir_101_GradCAMElementWise_01FP_Pos_505_p}&
      \img{images/CFP/sim/Adaface_ir_101_CorrRISE_01FP_Pos_505_g_sim}&
      \img{images/CFP/sim/Adaface_ir_101_CorrRISE_01FP_Pos_505_p_sim}&
      \img{images/CFP/sim/Adaface_ir_101_CorrRISE_01FP_Pos_505_g_dissim}&
      \img{images/CFP/sim/Adaface_ir_101_CorrRISE_01FP_Pos_505_p_dissim}&
      \img{images/CFP/sim/Adaface_ir_101_fggb_01FP_Pos_505_g_sim}&
      \img{images/CFP/sim/Adaface_ir_101_fggb_01FP_Pos_505_p_sim}&
      \img{images/CFP/sim/Adaface_ir_101_fggb_01FP_Pos_505_g_dissim}&
      \img{images/CFP/sim/Adaface_ir_101_fggb_01FP_Pos_505_p_dissim}&      
      \img{images/CFP/sim/Adaface_ir_101_fame_cos_01FP_Pos_505_g}&
      \img{images/CFP/sim/Adaface_ir_101_fame_cos_01FP_Pos_505_p}&
      \img{images/CFP/sim/Adaface_ir_101_fame_1-cos_01FP_Pos_505_g}&
      \img{images/CFP/sim/Adaface_ir_101_fame_1-cos_01FP_Pos_505_p}\\
      
      
  
      \end{tabular}
      }
  \Caption[fig:activations-fr]{Three dataset positive pairs}{
    The figure provides a comparative visualization of explanation maps generated on three representative datasets across different XAI teichniques. ARFace (scarf protocol), SCFace (medium distance), and CFP (frontal–profile protocol), for positive image pairs using different networks (AdaFace-34, AdaFace-50, and AdaFace-100) and multiple XAI techniques, including Grad-CAM, Grad-CAM Element-wise, CorrRISE (similar and dissimilar regions), and the proposed FAME with two complementary loss designs. 

  }

\end{figure*}


==> figures/tab_eval_fr.tex <==
\begin{table*}
  \Caption[tab:eval-fr-all]{Quantitative Evaluation of Face Recognition Attribution}{
    This table compares different XAI methods evaluated using the Delete ($\downarrow$) and Insert ($\uparrow$) metrics across multiple face recognition protocols.
    Three AdaFace-based backbones (IResNet18, IResNet50, IResNet101) are tested on three datasets: AR Face, SCface, and CFP with default evaluation protocols.\\
    \textcolor{red}{Note to the reviewers: experiments on FGGB are still running at submission deadline, please find their results in the supplemental material.}
    % \todo{Add FGGB}
  }
  \centering
  \tiny
  \begin{tabular}{|l|c||c|c|c|c|c|c||c|c|c|c|c|c||c|c|c|c|}
    % \toprule
    \hline
    && \multicolumn{6}{c||}{ARface} & \multicolumn{6}{c||}{SCface} & \multicolumn{4}{c|}{CFP}\\[.3ex]
    \cline{3-18}
    FR model& XAI&  \multicolumn{2}{c|}{neutral} & \multicolumn{2}{c|}{glass} & \multicolumn{2}{c||}{scarf} & \multicolumn{2}{c|}{close} & \multicolumn{2}{c|}{medium} & \multicolumn{2}{c||}{far}  & \multicolumn{2}{c|}{FF} &  \multicolumn{2}{c|}{FP}\\
    % \midrule
    \cline{3-18}
    & & Delete & Insert & Delete & Insert & Delete & Insert & Delete & Insert & Delete & Insert & Delete & Insert & Delete & Insert & Delete & Insert \\\hline
     \multirow{4}{*}{IResNet18}
    & Grad-CAM & 50.51 & 50.32 & 63.77 & 65.63 & 61.71 & 81.78 & 66.56 & 70.33 & 62.47 & 63.03 & 53.64 & 55.73 & 76.94 & 89.02 & 55.04 & 66.79 \\
    & Grad-CAM-EW & \rednum{50.47} & 52.48 & 54.35 & 84.80 & 57.42 & 90.96 & 58.17 & 85.90 & 55.95 & \rednum{78.74} & 51.88 & \rednum{60.90} & 64.51 & 95.45 & 52.31 & 78.54 \\
    & CorrRISE $e_+$ & \rednum{50.47} & 50.00 & 53.69 & 80.20 & 53.84 & 92.66 & \rednum{55.87} & 84.23 & \rednum{54.59} & 74.17 & \rednum{51.30} & 59.56 & 69.19 & 94.43 & 51.94 & 77.90 \\
    & FAME $e_+$ & \rednum{50.47} & \rednum{52.78} & \rednum{53.06} & \rednum{85.43} & \rednum{53.41} & \rednum{92.86} & 56.80 & \rednum{86.22} & 55.05 & 78.53 & 52.40 & 60.67 & \rednum{60.75} & \rednum{95.58} & \rednum{51.87} & \rednum{79.96} \\
    % & fame2 & 50.47 & 52.78 & 53.06 & 85.43 & 53.41 & 92.86 & 56.80 & 86.22 & 55.05 & 78.53 & 52.40 & 60.67 & 60.75 & 95.58 & 51.87 & 79.96 \\

    \hline \hline

    \multirow{4}{*}{IResNet50}
     & Grad-CAM & 50.90 & 50.81 & 75.23 & 75.21 & 68.85 & 78.29 & 69.62 & 75.81 & 63.00 & 67.12 & 54.63 & 57.34 & 79.11 & 88.60 & 70.09 & 83.29 \\
     & Grad-CAM-EW & \rednum{50.77} & 54.23 & 59.71 & 90.88 & 57.44 & 91.20 & 60.48 & 87.92 & 56.87 & 78.17 & 52.64 & 62.71 & 65.65 & 95.48 & 56.78 & 93.61 \\
     & CorrRISE $e_+$ & \rednum{50.77} & 50.00 & 59.55 & 91.18 & 55.07 & 92.64 & 60.07 & 88.62 & 56.30 & 76.53 & \rednum{52.06} & 60.20 & 72.68 & \rednum{96.27} & 55.69 & 94.68 \\
     & FAME $e_+$ & \rednum{50.77} & \rednum{55.00} & \rednum{56.85} & \rednum{91.75} & \rednum{54.46} & \rednum{92.84} & \rednum{58.31} & \rednum{88.94} & \rednum{56.17} & \rednum{78.97} & 53.43 & \rednum{63.14} & \rednum{62.20} & 96.00 & \rednum{54.84} & \rednum{95.05} \\
    %  & fame2 & 50.77 & 55.00 & 56.85 & 91.75 & 54.46 & 92.84 & 58.31 & 88.94 & 56.17 & 78.97 & 53.43 & 63.14 & 62.20 & 96.00 & 54.84 & 95.05 \\
    \hline \hline

    \multirow{4}{*}{IResNet101}
     & Grad-CAM & 50.64 & 50.60 & 72.62 & 77.89 & 69.48 & 80.50 & 71.27 & 75.40 & 67.64 & 69.86 & 54.51 & 54.40 & 86.41 & 91.94 & 74.91 & 85.21 \\
     & Grad-CAM-EW & \rednum{50.60} & 52.91 & 60.44 & 90.09 & 59.12 & 90.80 & 60.57 & 87.17 & 59.05 & 80.56 & 52.41 & 59.48 & 70.17 & 96.70 & 59.26 & 94.36 \\
     & CorrRISE $e_+$ & \rednum{50.60} & 50.00 & 58.39 & 91.24 & 55.52 & \rednum{93.43} & 58.59 & 86.78 & 57.35 & 80.35 & \rednum{51.38} & 58.79 & 86.46 & \rednum{96.81} & 56.31 & 96.07 \\
     & FAME $e_+$ & \rednum{50.60} & \rednum{54.06} & \rednum{56.12} & \rednum{92.07} & \rednum{55.13} & \rednum{93.43} & \rednum{58.10} & \rednum{88.22} & \rednum{57.19} & \rednum{82.02} & 52.73 & \rednum{60.15} & \rednum{65.70} & 96.71 & \rednum{55.82} & \rednum{96.24} \\
    %  & fame2 & 50.60 & 54.06 & 56.12 & 92.07 & 55.13 & 93.43 & 58.10 & 88.22 & 57.19 & 82.02 & 52.73 & 60.15 & 65.70 & 96.71 & 55.82 & 96.24 \\
    \hline

    \end{tabular}
\end{table*}

